Integer Vector Addition Systems with States

This paper studies reachability, coverability and inclusion problems for Integer Vector Addition Systems with States (ZVASS) and extensions and restrictions thereof. A ZVASS comprises a finite-state controller with a finite number of counters ranging over the integers. Although it is folklore that reachability in ZVASS is NP-complete, it turns out that despite their naturalness, from a complexity point of view this class has received little attention in the literature. We fill this gap by providing an in-depth analysis of the computational complexity of the aforementioned decision problems. Most interestingly, it turns out that while the addition of reset operations to ordinary VASS leads to undecidability and Ackermann-hardness of reachability and coverability, respectively, they can be added to ZVASS while retaining NP-completness of both coverability and reachability.

==> lower.tex <==
\section{Lower Bounds}




==> qsos.tex <==
\section{Missing Proofs from Section~\ref{sec:inclusion}}

In this section, we show that inclusion for \ZVAS \ is
$\mathsf{\Pi}_2^\P$-hard. To this end, we reduce from validity in
\emph{quantified systems of linear Diophantine equations with $k$
  alternations (QSLDE$_k$)}. Such a system is given as
%
\begin{align*}
  S: \forall \vec{x}_1 \exists \vec{x}_2 \cdots Q_k \vec{x}_k.
  A_1\vec{x}_1 + \cdots + A_k\vec{x}_k \sim_k \vec{c},
\end{align*}
%
where
%
\begin{itemize}
\item each $\vec{x}_i$ is a dimension-$n_i$ vector of first-order variables;
\item $A_i\in \zint^{m\times n_i}$ and $\vec{c}\in \zint^m$ for some $m>0$;
\item $Q_k=\exists$ and ${\sim}_k$ is $=$ if $k$ is even;
\item $Q_k=\forall$ and ${\sim}_k$ is $\neq$ if $k$ is odd; and
\item all numbers are encoded in unary.
\end{itemize}

\vspace*{0.25cm} \problemx{QSLDE$_k$} {A system $S$ of quantified linear
  Diophantine equations with $k$ alternations.} 
        {Is $S$ valid?}

\begin{proposition}
  \label{prop:qslde-hardness}
  For every $k>0$, QSLDE$_k$ is $\mathsf{\Pi}_k^\P$-hard.
\end{proposition}
The proof of this proposition is deferred to
Section~\ref{ssec:qslde}. As an intermediate step, we show that a
generalization of \textsc{SubsetSum} is complete for every level in
the polynomial-time hiearchy in Section~\ref{ssec:qsos}. We can now
prove hardness for inclusion between \ZVAS.

\begin{lemma}
  Inclusion for \ZVAS \ is $\mathsf{\Pi}_2^\P$-hard.
\end{lemma}
\begin{proof}
  Let $S: \forall \vec{x}.\exists \vec{y}.A\vec{x} + B\vec{y}=\vec{c}$
  be an instance of a quantified system of linear Diophantine
  equations such that $A$ and $B$ consist of column vectors
  $\vec{a}_1,\ldots,\vec{a}_m$ and $\vec{b}_1,\ldots,\vec{b}_n$,
  respectively. Let $\mathcal{A}$ be the \ZVAS \ consisting of a
  single state $q$ with self-loops adding
  $\vec{a}_1,\ldots,\vec{a}_m$, and let $\mathcal{B}$ be the \ZVAS
  \ consisting of a single state $p$ with self-loops adding
  $\vec{b}_1,\ldots,\vec{b}_m$ to the counter. The same reasoning as
  in Lemma~\ref{lem:zvas-reachability-hardness} clearly yields that
  $\mathit{reach}(\mathcal{A},q(\vec{c})) \subseteq
  \mathit{reach}(\mathcal{B},p(\vec{0}))$ if, and only if $S$ is
  valid, which together with Proposition~\ref{prop:qslde-hardness}
  yields the desired hardness result.\qed
\end{proof}
%
It is worth mentioning that it is not clear whether
$\mathsf{\Pi}_2^\P$-hardness for \ZVAS \ still holds when asking for inclusion
for fixed initial vectors, \emph{e.g.} for inclusion instances of the
form $\mathit{reach}(\mathcal{A},q(\vec{0})) \subseteq
\mathit{reach}(\mathcal{B},p(\vec{0}))$. It is easily seen that the
problem is \NP-hard, however it has resisted some serious attempts to
improve the lower bound. In particular, this problem is equivalent to
asking given two finite sets $A,B\subseteq \zint^d$ whether $\langle A
\rangle$, the semigroup generated by $A$, is a subsemigroup of
$\langle B \rangle$. We are not aware of any tight bounds concerning
this problem. 


\subsection{QSOS$_k$ is $\mathsf{\Pi}_k^\P$-complete}
\label{ssec:qsos}


The quantified sum of subset of order $k$ is following problem:
\vspace*{0.25cm}
\problemx{QSOS$_k$}
         {$M_1, \dots, M_k$ subsets of $\nat$, $T\in\nat$ a target number}
         {Is $\forall (M'_1 \subset M_1) \ \exists (M'_2 \subset M_2) \dots Q_k (M'_k \subset M_k) \ . \ \sum_{i=1}^k~\sum_{x\in M'_i}~x~\sim_k~T$ true ?}

where 
\begin{itemize}
\item $Q_k = \exists$ and $\sim_k$ denotes the equality between natural numbers respectively, when $k$ is even, 
\item $Q_k = \forall$ and $\sim_k$ denotes the inequality, when $k$ is odd. 
\end{itemize}



The quantified sum of subset with an arbitrary number of quantifier alternation is noted $QSOS$, and is proved \PSPACE-hard in \todo{cite}. Moreover, this proof can easily be extended to any level of the hierarchy.

\todo{can we write complete instand and prove only the hardness ? Stating that membership is trivial ?}
\begin{theorem}
The problem $QSOS_k$ is $\mathsf{\Pi}_k^\P$-hard.
\end{theorem}

\begin{proof}
To prove $\mathsf{\Pi}_k^\P$-hardness, there are two cases to consider: $k$ is even or odd. If it is even, $Q_k$ is an existential quantifier, $~_k$ is an equal symbol, and the proof is very similar to the proof of PSPACE-hardness, thus we give the detail of the reduction, but for correctness, the reader may refer to the original paper.

Given a formula $\varphi = \forall X_1 \exists X_2 \forall X_3 \dots \exists X_k . \ \bigwedge_{i=1}^m C_i$ where $C_i = z_{i_1} \vee z_{i_2} \vee z_{i_3}$. Let $N = \sum_{i=1}^m |X_i|$. Build the following instance:
$M_1, M_2, \dots, M_k \cup P, T$ where:
\begin{itemize}
\item $X_i = \{ x_1^i, \dots, x_{r_i}^i \}$
\item $M_i = \{ m_1^i, \dots, m_{r_i}^i \}$
\item $P = \{ n_j^i : i \in [k], j \in [r_i] \} \cup \{ c_1, \dots, c_m, d_1, \dots, d_m\}$
\end{itemize}
with numbers in base 10 (or whatver greater than 4):

\begin{align*}
m_j^i = \left( \underbrace{k_1k_2\dots k_m}_m \underbrace{0 \dots 0\stackrel{(i)}{1}0 \dots 0}_N \right) 
& \text{, \quad where $k_l$ is the number of occurences of literal $x_j^i$ in the $l$-th clause}\\
%%
n_j^i = \left( \underbrace{k_1k_2\dots k_m}_m \underbrace{0 \dots 0\stackrel{(i)}{1}0 \dots 0}_N \right) 
& \text{, \quad where $k_l$ is the number of occurences of literal $\neg x_j^i$ in the $l$-th clause} \\
%%
c_i = \left( \underbrace{0 \dots 0\stackrel{(i)}{1}0 \dots 0}_m \underbrace{0\dots 00 \dots 0}_N \right)
& \text{, \quad (balancing numbers)} \\
%%
d_i = \left( \underbrace{0 \dots 0\stackrel{(i)}{2}0 \dots 0}_m \underbrace{0\dots 00 \dots 0}_N \right)
& \text{, \quad (balancing numbers)} \\
T = \left( \underbrace{4 \dots 444 \dots  4}_m \underbrace{1\dots 111 \dots 1}_N \right)
& \text{, \quad (target number)}
\end{align*}


Obviously, $\varphi$ is true if and only if the following holds: $\forall M_1' \subseteq M_1 \ \exists M_2' \subseteq M_2 \dots \exists M_k' \subseteq (M_k \cup P) . \ \sum_{i=1}^k (\sum M_i) = T$. Indeed, the $N$ rightmost digits ensure that for any $i, j$, either $m_j^i$ or $n_j^i$ but not both are part of the sum, which encodes that $x_j^i$ is either set to true or to false. After the choice of the subsets of the $M_i$, the $k$ leftmost digits take values among $\{0,3\}$ depending on how many of their literals are set to true. The existential choice over $P$ then allows to add 1, 2 or 3 to these values to reach the value $4$ required by the target vector. 


If it is odd, we rather prove the dual result, hence we reduce the truth value of a formula $\varphi = \exists X_1 \forall X_2 \dots \exists X_k \ . \ \bigwedge_{i=1}^m C_i$ to the truth of the statement $\exists (M'_1 \subset M_1) \forall (M'_2 \subset M_2) \dots \exists (M'_K \subset M_k) \ . \ \sum_{i=1}^k \sum_{x \in M'_i} x = T$ for some $M_1, M_2, \dots, M_k, T$ that can be constructed in polynomial time from $\varphi$. The reduction is essentially the same, the $M_i$ for $i\in [k-1]$ non deterministically choose the true variable from $\varphi$, then the last set $M_k$ consistently complete with the right negative literals, and the balancing numbers to obtain the target number.

\qed
\end{proof}

Proving hardness for any level of the polynomial hierarchy was not much effort, but what we are really interested in is the hardness for the $\mathsf{\Pi}_2^\P$ class.

\begin{corollary} 
$QSOS_2$ is $\Pi_2^P$-hard
\end{corollary}


\subsection{Linear sets inclusion}

In section \ref{sec:inclusion}, we proved $\mathsf{\Pi}_2^\P$-hardness for \ZVAS \ inclusion by reduction from a quantified system of linear Diophantine equations, which we shall now prove $\mathsf{\Pi}_2^\P$-hard as well. We present a reduction from $QSOS_2$.

Given a $QSOS_2$ instance, $M_1 = \{ m_1, \dots, m_p \} \subset \nat, \ M_2 = \{ n_1, \dots, n_r \} \subset \nat$ and $T \in \nat$, we constuct an instance $A \in \zint^{d\times p}, B \in \zint^{d\times r + p + r}$, $\vec{c} \in \zint^d$ with $d = 1 + p + r$:

\begin{align*}
A = \left[
\begin{array}{ccc}
m_1&\cdots &m_p \\ \hline
&&\\
    &I_p & \\
&&\\ \hline
&&\\
& \vec{0} & \\
&&\\ 
\end{array}
\right]
%
B = \left[
\begin{array}{ccc|ccc|ccc}
n_1&\cdots &n_r&0&\dots &0 &0&\dots&0 \\ \hline
&&& &&& &&\\
    &\vec{0} &&& I_p &&& \vec{0}   &   \\
&&& &&& &&\\ \hline
&&& &&& &&\\
& I_r &&& \vec{0} &&& I_r & \\
&&& &&& &&\\ 
\end{array}
\right]
%
\vec{c} = \left[
\begin{array}{c}
T \\ \hline
1 \\
\vdots \\
1 \\ \hline
1 \\
\vdots \\
1 \\
\end{array}
\right]
\end{align*}


Any solution $\vec{x}$, $\vec{y}$ of this system can be decomposed in $\vec{x} = \vec{x_1}$ of size $p$ and $\vec{y} = (\vec{y_1}, \vec{x_1}, \vec{y_2})$ of respective size $r, p$ and $r$. All the dimensions except the first one enforces that $\vec{x_1}, \vec{x_2}, \vec{y_1}, \vec{y_2}$ takes values in $\{0,1\}$: indeed $\vec{x_1} + \vec{x_2} = \vec{y_1} + \vec{y_2}= (1\dots1)$. Therefore, in the first dimension equality $\sum_{i=1}^p m_i\vec{x}(i) + \sum_{i=1}^r n_i \vec{y}(i) = T$, the vectors $\vec{x}$ and $\vec{y}$ can be seen as the characteristic functions of $M_1$ and $M_2$ respectively, thus the linear system has a solution if and only if the $QSOS_2$ instance has a solution.

However, this reduction relies on a binary encoding of numbers in the matrices $A$ and $B$, indeed in the $QSOS_2$ instance, the natural numbers sets must be given in binary for the hardness proof to work. But for linear systems, the result may be strengthened: the problem is still $\mathsf{\Pi}_2^\P$-complete with a unary encoding. The idea is very common: we use dimensions to store the binary encoding of a number.

For readability, we give the instance as a system of equations, because the resulting matrices would be full of zeros and hard to understand. Let $q+1$ be the number of digits required to write in binary the greatest element of the sets $M_1$ and $M_2$. Every $m_i$ (resp. $n_i$) has a unique decomposition: $m_i = \sum_{j=0}^q m_{ij}2^j$. Matrices $A$ and $B$ (that won't be given explicitely) now have size $(1+(p+r)(q+2))\times((2+q+1)p)$ and $(1+(p+r)(q+2))\times((2+q+1)r)$. Variables are $(x_i, \bar{x}_i, x_{i0}, \dots, x_{iq})$ for $i \in [p]$, and $(y_i, \bar{y}_i, y_{i0}, \dots, y_{iq})$ for $i \in [r]$, and the $(1+p+p(q+1)+r+r(q+1))$ equations are:
\begin{align}
\left. \begin{array}{l}
  \sum_{i=0}^p x_{i0} + \sum_{i=0}^r x_{i0} = T  \\
\end{array} \right \} \quad &\text{1 equation} \label{one}\\
%
\left. \begin{array}{l}
x_i + \bar{x}_i = 1  \\
\end{array} \right \} \quad &\text{$p$ equations} \label{two}\\
%
\left. \begin{array}{ll}
  x_{iq} -  m_{iq} x_i = 0  \\
  x_{ij} - 2x_{i(j+1)} - m_{ij} x_i = 0   \\
\end{array} \right \} \quad &\text{$p(q+1)$ equations} \label{three}\\
%
\left. \begin{array}{l}
  y_i + \bar{y}_i = 1  \\
\end{array} \right \} \quad &\text {$r$ equations} \label{four}\\
%
\left. \begin{array}{ll}
  y_{iq} - n_{iq} y_i =0  \\
  y_{ij} - 2y_{i(j+1)} - n_{ij} y_i = 0  \\
\end{array} \right \}  \quad &\text{$r(q+1)$ equations} \label{five}
\end{align}

As in the previous reduction, equations \ref{two} and \ref{four} enforce the $x_i$ and $y_i$ to be $0$ or $1$. Equations in \ref{three} ensure that $x_{ij} = \sum_{k=j}^q m_{ik} x_i 2^{k-j}$, which in the ends give $x_{i0} = \sum_{k=0}^q m_{ik} x_i 2^k = m_i x_i$ (same for $y_{i0}$ with equation \ref{five}). This equality explains equation \ref{one}, which is actually the same constraint as in the previous reduction.





==> results.tex <==
\section{Results}




